Clustering of steady-state correlations in open systems with long-range interactions

Lieb-Robinson bounds are powerful analytical tools for constraining the dynamic and static properties of non-relativistic quantum systems. Recently, a complete picture for closed systems that evolve unitarily in time has been achieved. In experimental systems, however, interactions with the environment cannot generally be ignored, and the extension of Lieb-Robinson bounds to dissipative systems which evolve non-unitarily in time remains an open challenge. In this work, we prove two Lieb-Robinson bounds that constrain the dynamics of open quantum systems with long-range interactions that decay as a power-law in the distance between particles. Using a combination of these Lieb-Robinson bounds and mixing bounds which arise from "reversibility" -- naturally satisfied for thermal environments -- we prove the clustering of correlations in the steady states of open quantum systems with long-range interactions. Our work provides an initial step towards constraining the steady-state entanglement structure for a broad class of experimental platforms, and we highlight several open directions regarding the application of Lieb-Robinson bounds to dissipative systems.

==> arXiv submission/preamble.tex <==
% \usepackage[latin1]{inputenc}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{bm}
\usepackage{layout}
\usepackage{float}
\usepackage{amsfonts}
\usepackage{amssymb}%
% \usepackage[margin=0.75in]{geometry}
\usepackage{color}
\usepackage{soul}
\usepackage{mathtools}
\usepackage{varwidth}
\usepackage[colorlinks=true,citecolor=blue]{hyperref}
\theoremstyle{definition}
% \newtheorem{theorem}{Theorem}
\newtheorem{claim}{Claim}
\newtheorem{problem}{Problem}
% \newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{conjecture}{Conjecture}
% \newtheorem{corollary}{Corollary}
\usepackage[capitalise,compress]{cleveref}
\newcommand{\avg}[1]{\left \langle #1 \right\rangle}
\newcommand{\corrc}[1]{\left \langle #1 \right\rangle_c}
\newcommand{\ket}[1]{\left | #1 \right\rangle}
\newcommand{\oket}[1]{\left | #1 \right)}
\newcommand{\bra}[1]{\left \langle #1 \right |}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\smallfrac}[2][1]{\mbox{$\textstyle \frac{#1}{#2}$}}
\newcommand{\Tr}{\mathrm{Tr}}
\renewcommand{\Re}{\mathrm{Re}}
\newcommand{\braket}[2]{\left\langle #1|#2\right\rangle}
\newcommand{\bracket}[3]{\left\langle #1|#2|#3\right\rangle}
\newcommand{\proj}[1]{\ket{#1}\bra{#1}}
\newcommand{\abs}[1]{\left | #1 \right|}
\renewcommand{\epsilon}{\varepsilon}
\renewcommand{\O}[1]{ O\left(#1\right)}
%\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\lnorm}[1]{\left\|#1\right\|_l}
\newcommand{\comm}[1]{\left[#1\right]}
% \newcommand{\C}{\mathcal{C}}
\newcommand{\Laplace}{\mathcal{L}}
% \newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\arrowto}{$\Rightarrow$ }
\newcounter{para}
\newcommand{\dist}{\textrm{dist}}
\newcommand\observation{ \par\emph{Observation \refstepcounter{para}\thepara.\space}}
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\newcommand{\U}[2]{U^{#1}_{#2}}
\newcommand{\Udag}[2]{\left(U^{#1}_{#2}\right)^\dag}
\newcommand{\B}{\mathcal B}
\newcommand{\const}{\text{const.}}
%\renewcommand{\labelitemi}{--}
\makeatother
\newcommand{\nmax}{\omega_*}
\newcommand{\qmax}{q_{\text{max}}}
\newcommand{\ad}{\text{ad}}
\newcommand{\Hpl}{\mathbb{H}_{\alpha}}

\newcommand{\tr}{\text{Tr}}
% \newcommand{\mL}{\mathcal{L}}
% \newcommand{\mT}{\mathcal{T}}
% \newcommand{\mQ}{\mathcal{Q}}

%Packages/Commands Added by Adam%
\usepackage{braket}
\newcommand{\Z}{\mathbb{Z}}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\usepackage{array}
\newcolumntype{L}{>{$}l<{$}} % math-mode version of "l" column type
\newcolumntype{C}{>{$}c<{$}} % math-mode version of "c" column type
\newcolumntype{R}{>{$}r<{$}} % math-mode version of "r" column type

\usepackage{xcolor}
\newcommand{\minh}[1]{{\color{red} [Minh: #1]}}
\newcommand{\adam}[1]{{\color{red} [Adam: #1]}}

\usepackage{mathtools}
% \DeclarePairedDelimiter\ceil{\lceil}{\rceil}
% \DeclarePairedDelimiter\floor{\lfloor}{\rfloor}



%%% Allow cross-referencing of main.tex %%%
\usepackage{xr}
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother
\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}

% \newcommand{\Th}[1]{\Theta\left(#1\right)}

\usepackage{tikz}

\newcommand{\Li}{\text{Li}}
\newcommand{\Su}{\text{Su}}
\newcommand{\floorstar}[1]{\floor{#1}^*}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\Py}{\mathbb{P}_Y}
\newcommand{\length}{\text{length}}

